An Empirical Study of Token-based Micro Commits

In software development, developers frequently apply maintenance activities to the source code that change a few lines by a single commit. A good understanding of the characteristics of such small changes can support quality assurance approaches (e.g., automated program repair), as it is likely that small changes are addressing deficiencies in other changes; thus, understanding the reasons for creating small changes can help understand the types of errors introduced. Eventually, these reasons and the types of errors can be used to enhance quality assurance approaches for improving code quality. While prior studies used code churns to characterize and investigate the small changes, such a definition has a critical limitation. Specifically, it loses the information of changed tokens in a line. For example, this definition fails to distinguish the following two one-line changes: (1) changing a string literal to fix a displayed message and (2) changing a function call and adding a new parameter. These are definitely maintenance activities, but we deduce that researchers and practitioners are interested in supporting the latter change. To address this limitation, in this paper, we define micro commits, a type of small change based on changed tokens. Our goal is to quantify small changes using changed tokens. Changed tokens allow us to identify small changes more precisely. In fact, this token-level definition can distinguish the above example. We investigate defined micro commits in four OSS projects and understand their characteristics as the first empirical study on token-based micro commits. We find that micro commits mainly replace a single name or literal token, and micro commits are more likely used to fix bugs. Additionally, we propose the use of token-based information to support software engineering approaches in which very small changes significantly affect their effectiveness.

==> Makefile <==
#!/usr/bin/make -f

CP=cp
RM=rm -f
TARG=main
#TARG=main_latexdiff

.PHONY: all clean

all:$(TARG).pdf

.SUFFIXES: .pdf .tex .aux .bbl

.tex.pdf:
	@\
	aux=$(<:%.tex=%.aux);\
	$(CP) $$aux $$aux-;\
	pdflatex $<;\
	echo ========;\
	diff -q $$aux $$aux- > /dev/null;\
	if [ $$? -eq 0 ]; then\
		echo No need for second compile.;\
	else\
		bibtex $$aux;\
		echo ========;\
		$(CP) $$aux $$aux-;\
		pdflatex $<;\
		echo ========;\
		diff -q $$aux $$aux- > /dev/null;\
		if [ $$? -eq 0 ]; then\
			echo No need for third compile.;\
		else\
			pdflatex $<;\
		fi;\
	fi;\
	$(RM) $$aux-
	$(RM) $(TARG).{aux,log,blg,cut,out,xcp,gz,xcp}

clean:
	$(RM) $(TARG).{pdf,aux,log,blg,cut,out,xcp,gz,xcp}


==> codes/data-preparation/ex-commit.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% https://github.com/torvalds/linux/commit/53221e11c7a0e85004c1a28f74e4e173f098d262
%% \tiny
%% \scriptsize
%% \footnotesize
%% \small
%% \normalsize
%% \large
%% \Large
%% \LARGE
%% \huge
%% \Huge
%% ============================================================================
%% ============================================================================	

\begin{lstlisting}[caption={An example commit in Git}, label={code:ex-commit-in-git}, upquote=true, language=diff]
m-kondo experiments $ git show -U0
commit ae80a4266c65bcf3d94ca414730b9ac82cbb81b7
Author: MKmknd <kondo@ait.kyushu-u.ac.jp>
Date:    Tue Nov 15 12:03:05 2022 +0900

        small update in the violin script

diff --git a/experiments/violin.R b/experiments/violin.R
index 80457cf..afcb296 100644
--- a/experiments/violin.R
+++ b/experiments/violin.R
@@ -19 +19 @@ test = function(target){
-      'label_notag'='NoTag'
+      'label_notag'='NoLab'
@@ -76 +76 @@ test = function(target){
-   g <- g + scale_x_discrete(labels=c('All', 'Bug', 'Clean', 'NoTag'))
+   g <- g + scale_x_discrete(labels=c('All', 'Bug', 'Clean', 'NoLab'))
\end{lstlisting}



==> codes/discussion/add-include.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% - add #include to fix (linux): https://github.com/torvalds/linux/commit/ed2149acc5535417774fe28862ea68cf05cc800c
%% \tiny
%% \scriptsize
%% \footnotesize
%% \small
%% \normalsize
%% \large
%% \Large
%% \LARGE
%% \huge
%% \Huge
%% ============================================================================
%% ============================================================================	

\begin{lstlisting}[caption={Example commit diff retrieved from\\
  \protect\texttt{ed2149acc5535417774fe28862ea68cf05cc800c} in Linux.}, label={code:add-include}, upquote=true, language=diff]
@@ -40,0 +41 @@
+#include <linux/vmalloc.h>
\end{lstlisting}


==> codes/discussion/add-parameter.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% add parameter (linux): https://github.com/torvalds/linux/commit/f98fd44bebac6aa203eaf8a433d3a3ded374bae5
%% \tiny
%% \scriptsize
%% \footnotesize
%% \small
%% \normalsize
%% \large
%% \Large
%% \LARGE
%% \huge
%% \Huge
%% ============================================================================
%% ============================================================================	

\begin{lstlisting}[caption={Example commit diff retrieved from\\
  \protect\texttt{f98fd44bebac6aa203eaf8a433d3a3ded374bae5} in Linux.}, label={code:add-parameter}, upquote=true, language=diff, basicstyle=\tiny, numberstyle=\tiny]
@@ -225,0 +226 @@ static struct plat_serial8250_port rb532_uart_res[] = {
+               .type           = PORT_16550A,
\end{lstlisting}


==> codes/discussion/change-identifier.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% change identifier (camel): https://github.com/apache/camel/commit/b334321081245eff06cde3ec56cdebf782de5125
%% \tiny
%% \scriptsize
%% \footnotesize
%% \small
%% \normalsize
%% \large
%% \Large
%% \LARGE
%% \huge
%% \Huge
%% ============================================================================
%% ============================================================================	

\begin{lstlisting}[caption={Example ``replace identifier'' commit diff retrieved from\\
  \protect\texttt{b334321081245eff06cde3ec56cdebf782de5125} in Camel.}, label={code:change-identifier}, upquote=true, language=diff, basicstyle=\tiny, numberstyle=\tiny]
@@ -28 +28 @@ import org.junit.runner.RunWith;
-public class CamelHdfs2Test extends AbstractSpringBootTestSupport {
+public class CamelHdfsTest extends AbstractSpringBootTestSupport {
@@ -37 +37 @@ public class CamelHdfs2Test extends AbstractSpringBootTestSupport {
-                .module(inferModuleName(CamelHdfs2Test.class))
+                .module(inferModuleName(CamelHdfsTest.class))
\end{lstlisting}


==> codes/discussion/swapping.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% swapping (linux): https://github.com/torvalds/linux/commit/78c68e8f5cd24bd32ba4ca1cdfb0c30cf0642685
%% \tiny
%% \scriptsize
%% \footnotesize
%% \small
%% \normalsize
%% \large
%% \Large
%% \LARGE
%% \huge
%% \Huge
%% ============================================================================
%% ============================================================================	

\begin{lstlisting}[caption={Example commit diff retrieved from\\
  \protect\texttt{78c68e8f5cd24bd32ba4ca1cdfb0c30cf0642685} in Linux.}, label={code:swapping}, upquote=true, language=diff, basicstyle=\tiny, numberstyle=\tiny]
@@ -93,0 +94,2 @@ static void ipu_crtc_atomic_disable(struct drm_crtc *crtc,
+       drm_crtc_vblank_off(crtc);
+
@@ -100,2 +101,0 @@ static void ipu_crtc_atomic_disable(struct drm_crtc *crtc,
-
-       drm_crtc_vblank_off(crtc);
\end{lstlisting}


==> codes/rq3/camel-ex1.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% https://github.com/torvalds/linux/commit/53221e11c7a0e85004c1a28f74e4e173f098d262
%% \tiny
%% \scriptsize
%% \footnotesize
%% \small
%% \normalsize
%% \large
%% \Large
%% \LARGE
%% \huge
%% \Huge
%% ============================================================================
%% ============================================================================	

%\begin{lstlisting}[caption={Example commit retrieved from\\
%  \protect\url{https://github.com/apache/camel/commit/106eed7b98a2e59214c151adb74be75a27583786}.}, label={code:rq3-camel-ex1}, upquote=true, language=diff]
\begin{lstlisting}[caption={Example ``other'' commit diff retrieved from\\
  \protect\texttt{106eed7b98a2e59214c151adb74be75a27583786} in Camel. This an example of the smallest commit (a micro
  commit of 5
  tokens added--the () is considered one token) that
  can add a new function although such function does nothing.}, label={code:rq3-camel-ex1}, upquote=true, language=diff]
+    private SchemaHelper() {
+    }
+
\end{lstlisting}


==> figures/data-preparation/ex-commit.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% omni/micro-commits
%% ============================================================================
%% ============================================================================	

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\columnwidth]{./figures/data-preparation/p-ex-commit.pdf}
  \caption{ 
    An example commit in Git
  }
  \label{fig:data-pre:ex-commit}
\end{figure}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> sections/old_sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Small changes\reb{, \eg, one-line changes,} are frequent in software development~\cite{purushothaman2005TSE}. 
For example, Alali~\et~\cite{alali2008ICPC} reported that approximately 19.9\% of commits in the GNU gcc system change at most five lines. 
Also, we found that 8.4\% of commits in the Linux kernel repository changed only a single code line (\sec{sec:motivation}). 
It is extremely likely that changes that add or remove a few tokens are for maintenance purposes, since adding a new
functionality is unlikely to be possible in a few tokens.
In this study, we call commits that change an extremely small number of tokens \textit{micro commits}.
\lis{code:ex-micro-commit} shows an example of a micro commit that adds one token.
If micro commits are common, it is important to understand their characteristics and the reasons for their creation,
specifically considering that, if they are common, the amount of effort invested in creating these commits is
significant.


Improving code quality is an ultimate goal for software engineering researchers, and several approaches have been widely
studied so far, such as automated program repair (APR), defect prediction, and fault localization. A good understanding
of the characteristics of micro commits can support such approaches, as it is likely that micro commits are addressing
deficiencies in larger commits; thus, understanding the reasons for creating micro commits are created can help understand the types of errors
that larger commits introduce.


While prior studies~\cite{purushothaman2005TSE,hindle2008MSR,alali2008ICPC} use churn (number of lines added and
removed) to characterize commits, this definition has a critical limitation:
they consider the line the finest-grained changed source code entity.
More specifically, such a definition loses information about changes in a line~\cite{german2019EMSE,meng2013ICSM,servant2017ICSE}. 
Another problem is that splitting or joining a line of code that is being changed results in noise.
For example, even if we split a line as a format change, this would be a change with multiple lines in the version control systems (e.g., Git), and it would be noise to analyze the history of the development process. 

This limitation causes researchers to fail to properly quantify the changes in micro commits.  For example,
\lis{code:ex-missed-micro-commit} shows a commit in the Linux repository that changes a few lines (\ie, three added and
two deleted lines).  While this commit corresponds with a multiple-lines change, it only adds a token ``static'' and is
a micro commit similar to \lis{code:ex-micro-commit}.  By studying the actual tokens changed in micro commits (instead
of the lines that they changed), one can get a much better understanding of the actual change performed by such commits.

\emph{Just-in-time (JIT) defect prediction approaches} frequently measure commits' numerical
features (\eg, number of files changed and number of added, removed, or changed lines) and predicts defective ones with machine learning classifiers~\cite{kamei2013TSE,kondo2020EMSE,kondo2019EMSE,hassan2009ICSE}.
Prior studies~\cite{kondo2020EMSE,mcintosh2018TSE} have reported that these approaches rely primarily on the
number of changed lines. Considering tokens instead of lines might bring new insights into these methods.
%\dmg{I removed this because we do not even argue whether small commits are buggy or not: thus they difficulty distinguishing defective and non-defective in very small commits.}
%\masa{Thanks!}


In this paper, we empirically investigate the characteristics of micro commits. First, we empirically define micro commits
as those that add at most five tokens \reb{and} remove at most five tokens
%to be commits that add 5 tokens and/or remove at most 5 tokens
(replacing a token would imply one removal and one addition). We then investigate the frequency, 
features, and purpose of micro commits in four well-known OSS projects written in Java and C. Specifically, we answer the
following research questions (RQs). \reb{We have also provided a summary of the key findings for each RQ. The detailed results are described in \sec{sec:rq1}, \sec{sec:rq2}, and \sec{sec:rq3}.}

\begin{itemize}
\setlength{\leftskip}{0.3cm}
\item[RQ1:] \textbf{\RQone{}}
	\\
	\textit{Motivation:}
		% To define token-based micro commits, we first investigate the quantitative characteristics of \textit{\oneLine{}s}, which is our definition of line-based micro commits, to decide the threshold in terms of tokens.
		% Based on the result, we define token-based \textit{micro commits} (hereafter, micro commits) that cover \oneLine{}s. 
		To define micro commits, we first turn our attention to \textit{\oneLine{}s}, which replace one line of
                code with another.
                Since \oneLines provide the minimal amount of change using traditional diff tools,
                they can be considered a valid upper threshold for the size of micro commits.
	\\
  \textit{Results:}
		Most \oneLine{}s add or remove at most five tokens (approximately 89--93\%).
		%Therefore, we define a micro commit as adding and removing at most five tokens in the same
		Therefore, we define a micro commit as \reb{adding at most five tokens and removing at most five tokens} in the same file. Furthermore, in the projects under study, between 6.8 and 16.5\% of all commits are
                micro commits. Commits that only replace one-token occurred between 2.4 and 5.2\% of
  all commits.

\item[RQ2:] \textbf{\RQtwo{}}
	\\
	\textit{Motivation:}
	This research question aims to explain their qualitative (the types of tokens/tokens they contain) and quantitative
        characteristics (how frequent they are and how many types of tokens/tokens they modify).\\
   \textit{Results:}
	Most micro commits replace a single token with one of the same types, and this token type is mostly an
        identifier name or a constant literal.
        Java and C differ on the most frequent tokens in micro commits.

      \item[RQ3:] \textbf{\RQthree{}}

	\textit{Motivation:}
		We intend to understand the purpose of micro commits (\eg, changing control flow, replacing the name of
                a variable, and modifying an expression) and whether a micro commit performs one or more activities.
		Specifically, we (1) classify the type of maintenance activity micro commits perform to understand their
                purpose and (2) manually inspect the changes applied to the source code to understand the purpose behind the micro commit.
	\\
  \textit{Results:}
		Almost half of micro commits are classified into defect-fixing activity.
		More than 90\% of micro commits apply a single operation to a single entity. 

\end{itemize}


The main contributions of this paper are as follows:
\begin{itemize}
%\item We propose the concept of micro commits as commits that at most add 5 tokens and/or replace 5 tokens, and
\item We propose the concept of micro commits as commits that \reb{add at most five tokens and remove at most five tokens} in the same file, and
  demonstrate that these types of changes are common.  
\item We empirically investigate micro commits and understand their quantitative and qualitative characteristics. We
  especially shed light on the purpose of micro commits (\ie, defect-fixing activity) with our manual inspection.

\item We propose the use of token-level information in the use of micro commits to support software engineering
  approaches that use extremely small changes (\eg, defect repair and defect prediction).
\item We provide the replication package of this study that contains a set of micro commits that have been manually labeled
  according to their purpose.
\end{itemize}


The organization of our paper is as follows:
\sec{sec:motivation} introduces motivating examples.
\sec{sec:dataset} explains our studied dataset. 
\sec{sec:rq1}, \sec{sec:rq2}, and \sec{sec:rq3} present the experiments and results based on our RQs.
% \sec{sec:results} presents the results of our case study.
%\sec{sec:discussion} discusses these results and shows takeaway messages.
%\sec{sec:discussion} introduces example micro commits and shows takeaway messages.
\sec{sec:discussion} proposes the use of token-level information.
\sec{sec:threats} describes the threats to the validity of our case study.
\sec{sec:related} introduces related work.
\sec{sec:conclusion} presents the conclusion.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/old_sections/rq1.tex <==
\section{\RQone}
\label{sec:rq1}

\subsection{Approach}

% What is a micro-commit? Informally, we define a micro-commit as a commit to source code that only modifies a very small
% section of the source code, such that this change is either preventing maintenance (removes a potential bug), active
% maintenance (fixes a known bug) or a non-functional change (i.e. comments, removal of dead code, etc). Our basic
% assumption is that, in a micro commits it is impossible to make any other type of maintenance activity.

What is a micro commit?
Informally, we define a micro commit as a commit to the source code that only modifies a small code fragment for maintenance purposes, such as preventive maintenance (\eg, removing a potential bug), active maintenance (\eg, fixing a known bug), or a non-functional change (\eg, comments and removal of dead code).

Ideally, we would like to define a micro commit in terms of the number of tokens it adds, removes, or changes. Given that version
control systems can only identify additions and removals, we can define a micro commit as a change that adds or
removes at most N tokens, where N is a small number. The challenge becomes the identification of the ideal size for N.

For this purpose, we turn our attention to \oneLine{}s.
%We define a \oneLine as a commit that has the following property:
We define a \oneLine{} as a commit with the following property:
% \emph{the commit has exactly one hunk, and this hunk is composed of a line removed, and one line inserted} (we ignore changes to comments).
\emph{the commit has exactly one hunk, which is composed of one line removed and one line added}.
% Thus, a \oneLine corresponds to a change to one line of source code that already exists (and does not include moving, inserting, nor deleting a line of code), and we assume that one-line commits can only perform the same types of
Thus, a \oneLine{} corresponds to a change to one existing line of source code that already exists and does not include
moving, inserting, or deleting such a line of code.
%Also, we assume that \oneLine{}s can only perform the same types of activities that micro commits (\ie, preventing and active maintenance and non-functional changes).
We want micro commits and \oneLine{}s to change a similar amount of code (an extremely small one). Thus, we use the number
of tokens changed in most \oneLine{}s as a way to determine the ideal size in tokens of a micro commit. In this manner,
we can assume that both \oneLine{}s and micro commits perform 
the same types of maintenance operations.
% Thus, by measuring the number of tokens in \oneLine{}s, we can identify the ideal size of a micro commit.

Our methodology can be summarized as follows: we start by 
identifying \oneLines using the line-based diffs (as described in the previous section). We then analyze the corresponding token-based diffs 
to identify the number of tokens that are added and removed in each of these commits.

\subsection{Results}


% \begin{table}[htbp]
%   \centering
% \begin{tabular}{lrrr}
% \hline
% Project & \oneLines & Commits & Prop (\%)\\
% \hline
% Camel & 2405 & 38458 & 6.3\\
% Hadoop & 2302 & 53796 & 4.3\\
% Linux & 62591 & 748618 & 8.4\\
% Zephyr & 1924 & 22097 & 8.7\\
% \end{tabular}
%   \caption{Number of \oneLines}
%   \label{tab:oneLineCounts}
% \end{table}

\input{figures/rq1/heatOneLineTokens}
\input{figures/rq1/token1lAccum}
\input{figures/rq1/heatTokens}



\textbf{Approximately 90\% of One-line commits consist of at most five tokens.}
%Table~\ref{tab:oneLineCounts} shows the number of \oneLines. As it can be observed, there are a significant number of these
\tab{tab:motivation:micro-commits} shows the number of \oneLines.
%As it can be observed, there are a significant number of these commits in these projects (between 4.3 and 8.7\% of all source code commits). 
As described in \sec{sec:motivation}, there are a significant number of these commits in the studied projects (4.28--8.71\%).
Figure~\ref{fig:oneLineHeat} shows the proportion of \oneLine{}s according to the number of tokens that they
have added and removed between 0 and 10. As can be seen, the majority of these commits add or remove at most five tokens. 
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp40/08_kondo.sh (label: exactly_one_token_in_one_line_commits)
%% ============================================================================
%% ============================================================================	
There are a significant number of \oneLines that remove and add exactly one token (between approximately 45 and 60\% of all \oneLine{}s).
%There are a significant number of \oneLines that remove and add exactly one token (between 42 and 55 percent of all \oneLine{}s).
Figure~\ref{fig:oneLineAccum} shows the accumulated distribution of \oneLines according to the maximum number of
tokens they add or remove.
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp40/09_kondo.sh 
%% exp40/data/maxtokenadded.csv
%% ============================================================================
%% ============================================================================	
As can be seen, between approximately 55\% and 64\% add-or-remove at most one token, between 76\% and
82\% add-or-remove at most three tokens, and between 89\% and 93\% add-or-remove at most five tokens.


\textbf{A large proportion of ``all'' commits also add or remove at most five tokens. }
Figure~\ref{fig:allHeat} shows the proportion of ``all'' commits according to the number of tokens they add and remove between 0 and 10.
Note that most of these commits also fall between zero and five.
%Therefore, we \textbf{define a micro commit as a commit that adds-or-removes at most five tokens, comments excluded}.
Therefore, we \textbf{define a micro commit as a commit that \reb{adds at most five tokens and removes at most five tokens} in a file}.
Because One-line commits fix only one file, we use both the number of tokens condition and the number of files condition. 
As shown in \figs{fig:oneLineHeat} and \ref{fig:allHeat}, commits that replace exactly one token (\ie, one added and one removed)
are a significant type of micro commit. As shown in \tab{tab:micro}, between 6.75\% and 16.50\% of commits are
micro commits, and approximately 1 in 3 micro commits are one-token commits in all projects. 
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp40/08_kondo.sh  (label: echo "one line" and echo "two lines")
%% ============================================================================
%% ============================================================================	
As expected, most of these commits modify a few lines: between 59.92\% and 64.09\% modify add or remove at most one line, and between 66.83\% and 74.52\%
add-or-remove two lines.

% By defining micro commits in terms of tokens we can analyze
% multiple-line commits that have modified very few tokens, thus increasing the confidence that micro commits are not
% adding functionality to their corresponding projects.

\input{tables/rq1/micro-onetoken-commit}

%\begin{hassanbox}{\columnwidth}
%\end{hassanbox}
\summarybox{Summary of RQ1}
{
  Approximately 90\% of \oneLines add or remove at most five tokens. 
  Based on this result, we define a micro commit as a commit that \reb{adds at most five tokens and removes at most five tokens} (\ie, the maximum size is five added and five deleted tokens) in a file. 
  In the projects under study, micro commits are a significant proportion of all 
  source code commits (between 6.75 and 16.50\%), and between 2.39 and 5.18\% of commits replace exactly one token.
  Approximately 90\% of \oneLines are micro commits.
}

  %%% Local Variables:
  %%% mode: latex
  %%% TeX-master: "../main"
  %%% End:


==> sections/old_sections/rq3.tex <==
\section{\RQthree{}}
\label{sec:rq3}


\input{tables/rq3/swanson-category.tex}

\subsection{Approach}

This RQ aims to understand the details of the maintenance activities performed by micro commits, although RQ2 explains the quantitative and qualitative characteristics.
Specifically, we investigate the purpose of micro commits and whether a micro commit performs one or more activities.
We call the former \emph{high-level maintenance activities} and the latter \emph{low-level maintenance activities}. 
Such an understanding gives us insight into whether understanding micro commits can support several approaches in software engineering (see the details in \sec{sec:discussion}).

We provide two perspectives to answer this research question:

\begin{enumerate}
\item We classify micro commits into high-level maintenance activities defined by Swanson~\cite{swanson1976ICSE}: \textit{corrective}, \textit{adaptive}, and \textit{perfective}.
The details of each category are described in \tab{tab:rq3:swanson-category}.
\item We manually inspect a large set of micro commits to identify the types of low-level activities each commit performs.
\end{enumerate}


\subsubsection{Classifying micro commits into high-level maintenance activities}

To classify commits into high-level maintenance activities, we 
followed the methodologies used in prior studies~\cite{mockus2000ICSM,purushothaman2005TSE}, which use keywords in commit messages to classify micro commits.
More specifically, if at least one of the keywords is included in the commit messages, we classify the commit into that category.
Otherwise, we do not label commits. 
We used the keyword list defined by Levin~\et~\cite{levin2016ICSME} as follows:
\emph{corrective}$=$\{``fix'', ``esolv'', ``clos'', ``handl'', ``issue'', ``defect'', ``bug'', ``problem'', ``ticket''\},
\emph{adaptive}$=$\{``add'', ``new'', ``introduc'', ``implement'', ``implemented'', ``extend'', ``feature'', ``support''\}, and
\emph{perfective}$=$\{``refactor'', ``re-factor'', ``reimplement'', ``re-implement'', ``design'', ``replac'', ``modify'', ``updat'', ``upgrad'', ``cleanup'', ``clean-up''\}.


\reb{
The detailed procedure is as follows.
\begin{stepitemize}
\item[\textbf{Step 1:}] 
  Apply preprocessing to the commit messages using the NLTK package\footnote{\url{https://www.nltk.org/}} in Python by following the steps below:
  \begin{itemize}
    \item
    Tokenize the text and convert all words to lowercase.
    \item
    Remove stopwords and punctuation.
    \item
    Perform stemming on all words.
  \end{itemize}
\item[\textbf{Step 2:}]
   Check if the stemmed commit message contains a keyword for each category.
 \item[\textbf{Step 3:}]
    Classify each commit into categories based on keywords present in the commit message.
\end{stepitemize}
}


Because the maintenance activity described above is high-level, this classification overlooks low-level activities.
This high-level classification shows that micro commits generally correspond to defect-fixing commits.
This result implies that empirically analyzing micro commits can contribute to software engineering research, such as APR and defect prediction.
Hence, we performed a manual inspection to understand the low-level activity that the micro commits performed as the second perspective. 

\subsubsection{Classifying micro commits into low level maintenance activities}

We manually inspect the micro commits to understand what types of change were performed from a source code perspective, considering removed and/or added tokens.

Our manual inspection consisted of two phases: (1) \textit{\reb{constructing a coding guide}} and (2) \textit{manual classification}. 
\reb{Constructing a coding guide for manual classification/annotation is a common practice in the field of mining software repositories~\cite{hata2019ICSE,wang2021EMSE,chouchen2021SANER,hata2022EMSE,wang2023EMSE,zanaty2018ESEM}. To create the coding guide, we referred to previous studies~\cite{hata2019ICSE,wang2021EMSE,chouchen2021SANER,hata2022EMSE,wang2023EMSE,zanaty2018ESEM} and followed the process detailed below.}


\reb{The initial coding guide was first discussed by the first and second authors. Since this is the first study to classify micro commits, we examined both micro commits and other types of commits to develop the initial coding guide. After constructing the initial coding guide, we aimed to reach a consensus among the first three authors for this guide and refine the guide. Specifically, we independently annotated 20 micro commits from a subset of all micro commits\footnote{This subset consists of micro commits that only change less than or equal to five tokens in main files (.c or .java files) in the Linux, Hadoop, and Zephyr projects to investigate a single operation commit for refining the coding guide.}.
We computed the agreement rate for these 20 micro commits using Fleiss' Kappa~\cite{fleiss1971} that is used to demonstrate inter-rater agreement when there are more than two raters. It is also frequently applied in the field of mining software repositories~\cite{chouchen2021SANER,hata2022EMSE}.
The Kappa coefficient is commonly interpreted using the following scale~\cite{viera2005}:
Slight agreement ($0.01 \leq k \leq 0.20$),
Fair agreement ($0.21 \leq k \leq 0.40$),
Moderate agreement ($0.41 \leq k \leq 0.60$),
Substantial agreement ($0.61 \leq k \leq 0.80$),
Almost perfect agreement ($0.81 \leq k \leq 0.99$).
Then we discussed the coding guide along with any inconsistencies in categorization to reach a consensus. We repeated this process until our categorization substantially matched, indicating that our coding guide was successfully constructed. We, therefore, repeated this process three times (\ie, independently classifying 60 commits). Finally, our agreement rate reached that point. \tab{tab:rq3:final-kappa} shows all agreement rates across three authors on the final 20 commits.}
\masa{need to update the kappa value}

\input{tables/rq3/kappa.tex}

\reb{Through this process, we identified two perspectives: \emph{operation} and \emph{entity}.
The operation indicates what kind of operations are applied, such as adding a new statement or changing an expression; the entity indicates source code elements where the operation is applied, such as expressions.
%This suggests that we classify micro commits according to the operations they involve (\eg, addition) and the entities to which these operations are applied (\eg, statement).
The details of the coding guide are described below.}

\reb{We utilized the following coding guide to categorize micro commits from the operations.}
\begin{itemize}
  \item \reb{\emph{add:} This refers to operations that add a completely new entity, including control flows.}
  \item \reb{\emph{replace:} This refers to operations that modify an entity, including control flows.}
  \item \reb{\emph{remove:} This refers to operations that completely remove an entity, including control flows.}
  \item \reb{\emph{multi:} This code indicates that multiple operations are applied.}
  \item \reb{\emph{no:} This code indicates that no functional change is applied.}
\end{itemize}


\reb{We utilized the following coding guide to categorize micro commits from the entities.}
\begin{itemize}
  \item \reb{\emph{identifier:} This refers to commits that only modify identifiers, such as variable names. If other entities, such as parentheses, are included, it would not be identified as an identifier but could be considered an expression.}
  \item \reb{\emph{statement:} This refers to commits that modify a complete statement, including the semicolon (;), such as an entire function call with its semicolon. The include directive statement is also regarded as a statement.}
  \item \reb{\emph{constant:} This refers to commits that only modify literals, such as strings. If other entities, such as parentheses, are included, it would not be identified as a constant but could be considered an expression.}
  \item \reb{\emph{declaration:} This refers to commits that modify declarations, such as variable declarations. However, if the commit can be classified as ``identifier'' or ``constant'', it should be categorized under these two categories rather than ``declaration''.}
  \item \reb{\emph{control flow:} This refers to commits that modify the control flow of execution, such as adding a new ``else'' statement.}
  \item \reb{\emph{expression:} If a commit does not match other categories and involves modifying a part of a statement, it would be classified into this category. Additionally, this category includes transformations from constants to variables or vice versa, as well as conversions from a variable to a pointer and vice versa.}
  \item \reb{\emph{multi:} This code suggests that operations are performed on multiple entities.}
  \item \reb{\emph{no:} This code indicates that no functional change is applied.}
\end{itemize}

\input{tables/rq3/manual-coding-result.tex}
\input{codes/rq3/linux-ex1.tex}
\input{codes/rq3/linux-ex2.tex}


\reb{\tab{tab:rq3:manual-coding-result} shows the summary and examples.
This represents different types of low-level maintenance activities performed by micro commits.
Let us describe two example commits. Listing~\ref{code:rq3-ex1} shows an example commit. This commit changes a function call and its argument.
More specifically, the identifiers of the function call and the argument value are replaced so that we classify this commit as operations$=$replace, and entities$=$identifier.
The commit of Listing~\ref{code:rq3-ex2} replaces an expression ``$++$'' into ``$--$''.  Hence, we classify this commit as operations$=$replace, and entities$=$expression.}


Because our agreement rate \reb{based on our coding guide} is nearly perfectly matched (\tab{tab:rq3:final-kappa}) and we made an internal consensus of \reb{the coding guide}, only the first author manually classified the 383 micro commits, similar to~\cite{wang2021EMSE,wang2023EMSE,hata2019ICSE,hata2022EMSE}. 
All our manual categorizations are available in our sheet%
\footnote{\texttt{https://docs.google.com/spreadsheets/d/1LmJdX2OSxfNYosEfydXVzhik3XaurqOjC49}\newline\texttt{BG4CWzug/edit?usp=sharing}}. \masa{need to update later}
The sample size in manual inspection was determined as a statistical representative with a confidence level of 95\% and a confidence interval of 5 for 130,578 micro commits from all studied projects.\footnote{\url{https://www.surveysystem.com/sscalc.htm}}

\subsection{Results}

\subsubsection{Classifying micro commits into high-level maintenance activities}

\input{figures/rq3/swanson-categorization}


\textbf{Micro commits are more likely to be defect-fixing activity than other commits.}
\fig{fig:rq3:swanson} shows the proportion of commits for each maintenance category.
In this figure, we compare the tendency of micro commits (dark gray) and all commits (light gray).
While adaptive and perfective micro commits are smaller than all commits except for one case, corrective micro commits are larger.
Also, these proportions are larger than all proportions in the other categories.
Hence, micro commits distinguishably correspond to the corrective commits.
This result shows that micro commits are usually applied to the source code to fix defects. 


\subsubsection{Classifying micro commits into low-level maintenance activities}


\input{tables/rq3/single-multi-matrix}
\input{tables/rq3/single-activity}



\input{codes/rq3/linux-ex4}

\textbf{Micro commits usually perform a single operation (90\%). Micro commits with multiple operations account for the remaining 10\%, and they correspond to two operations, but not more.}
\tab{tab:rq3:sin-mul-matrix} lists the proportion of micro commits classified into ``multi'' in the operation and entity.
Approximately 90\% of micro commits are classified into single operations (\ie, non ``multi''); thus, micro commits usually modify an extremely small section.
We refer to such commits as \textit{single-operation micro commits} (\eg, Listing~\ref{code:ex-single-token-modification} is a replace identifier).
We surprisingly observe that approximately 10\% are classified into \textit{multi-operation micro commits} (\ie, ``multi'').
Hence, multi-operation micro commits are also important for developers.
Listing~\ref{code:rq3-ex4} shows an example of a multi-operation micro commit.
This commit has a replace declaration and an add statement. 
It should be noted that such multi-operation micro commits have two operations only but not more; thus, at least in our manual inspection, micro commits having more than two operations do not exist. 

\input{codes/rq3/camel-ex1}

\textbf{Approximately 83.2\% of single-operation micro commits replace existing tokens.}
\tab{tab:rq3:single-activity} summarizes the frequency of the combination of operations and entities in single-operation micro commits.
The top-4 combinations include the ``replace'' operation, accounting for approximately 78.9\% (273/346).
Also, all the ``replace'' operation commits account for 83.2\% (288/346). 
This result suggests that many single-operation micro commits modify the existing source code, but do not add or remove the source code.
Note that, we found a single-operation micro commit that does not match our categorization, which is classified into ``other.''
Listing~\ref{code:rq3-camel-ex1} shows the micro commit.
This commit adds an empty method in a class in a Java file.
While adding a new method seems to contradict our assumption that micro commits cannot add functionality, this empty
method does nothing, even if called, and is therefore a non-functional change.
%Hence, we deduce that this commit is also included in our assumption.


\textbf{Multi-operation micro commits more frequently add-and-remove statements rather than single-operation ones.}
\tab{tab:rq3:multi-unique-activity} summarizes the frequency of the combination of operations and entities in multi-operation micro commits, and \tab{tab:rq3:multi-activity} summarizes the frequency of the pair of their combination for each commit.
The main difference from single-operation micro commits is that the ``add statement'' and the ``remove statement'' are top-2 and -3 (\tab{tab:rq3:multi-unique-activity}).
The reason is that multi-operation micro commits that add and remove statements appear most frequently (\tab{tab:rq3:multi-activity}).
This type of commit is used to move the statements, and therefore, 
change the order of execution and potentially the control flow of the program.
For example, Listing~\ref{code:rq3-ex3} shows an example micro commit.
This commit adds and removes a statement and changes the order of execution of the free statement to fix a bug related to freeing data.
This swapping activity is frequently observed in multi-operation micro commits. 

\input{tables/rq3/multi-activity-unique}
\input{tables/rq3/multi-activity}


\input{codes/rq3/linux-ex3}

\summarybox{Summary of RQ3}
{
Micro commits are most frequently classified into the ``corrective'' maintenance category, and this proportion is distinguishably larger than the other commits.
More than 90\% of micro commits apply a single operation to a single entity, and they mainly replace existing entity.
Multi-operation micro commits frequently change the order of statements. 
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/data-preparation/dataset-table.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% ============================================================================
%% ============================================================================	

% \begin{table}[t]
\begin{table}
    \caption{
        The list of columns in the table corresponding to commits in line or token repositories
}
\label{tab:data-pre:dataset-table}
\begin{center}
\scalebox{1.0}{
    \begin{tabular}{ccl}
    \toprule
    \multicolumn{1}{c}{Line table} & \multicolumn{1}{c}{Token table} & \multicolumn{1}{c}{Column}\\
    \midrule
    $\bigcirc$ & $\bigcirc$ & commit hash in line repository \\
    $\bigcirc$ & $\bigcirc$ & commit hash in token repository\\
    $\bigcirc$ & $\bigcirc$ & number of chunks               \\
    $\bigcirc$ & $\bigcirc$ & number of files                \\
    $\bigcirc$ &            & number of added lines          \\
               & $\bigcirc$ & number of added tokens         \\
    $\bigcirc$ &            & number of deleted lines        \\
               & $\bigcirc$ & number of deleted tokens       \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
\end{table}





==> tables/rq3/swanson-category.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% check the swanson paper
%% ============================================================================
%% ============================================================================	


% \begin{table}[t]
\begin{table}[t]
    \caption{
     Swanson's maintenance activity~\cite{swanson1976ICSE}
}
\label{tab:rq3:swanson-category}
\begin{center}
\scalebox{0.9}{
    \begin{tabular}{ll}
    \toprule
		\multicolumn{1}{c}{Category} & \multicolumn{1}{c}{Description}\\
    \midrule
    Corrective & Correcting failures\\
    Adaptive   & Adapting source code into changes (\eg, external environment)\\
    Perfective & Maintenance for non-functional features\\
    \bottomrule
    \end{tabular}
    }
    \end{center}
\end{table}







